Implicit Pairs for Boosting Unpaired Image-to-Image Translation

In image-to-image translation the goal is to learn a mapping from one image domain to another. In the case of supervised approaches the mapping is learned from paired samples. However, collecting large sets of image pairs is often either prohibitively expensive or not possible. As a result, in recent years more attention has been given to techniques that learn the mapping from unpaired sets. In our work, we show that injecting implicit pairs into unpaired sets strengthens the mapping between the two domains, improves the compatibility of their distributions, and leads to performance boosting of unsupervised techniques by over 14% across several measurements. The competence of the implicit pairs is further displayed with the use of pseudo-pairs, i.e., paired samples which only approximate a real pair. We demonstrate the effect of the approximated implicit samples on image-to-image translation problems, where such pseudo-pairs may be synthesized in one direction, but not in the other. We further show that pseudo-pairs are significantly more effective as implicit pairs in an unpaired setting, than directly using them explicitly in a paired setting.

==> abstract.tex <==
In image-to-image translation the goal is to learn a mapping from one image domain to another. In the case of supervised  approaches the  mapping is learned from  paired samples. However, collecting large sets of image pairs is often either prohibitively expensive or not possible.
As a result, in recent years more attention has been given to techniques that learn the mapping from unpaired sets.

In our work, we show that injecting implicit pairs into unpaired sets strengthens the mapping between the two domains, improves the compatibility of their distributions, and leads to performance boosting of unsupervised techniques by over 14\% across several measurements. 

The competence of the implicit pairs is further displayed with the use of pseudo-pairs, i.e., paired samples which only approximate a real pair. We  demonstrate  the  effect  of  the  approximated implicit samples on image-to-image translation problems, where such pseudo-pairs may be synthesized in one direction, but not in the other. We further show that pseudo-pairs are significantly more effective as implicit pairs in an unpaired setting, than directly using them explicitly in a paired setting.

==> figures/distributions_no_smiling_test.tex <==

% % 2x2 format on two columns
% \begin{figure}
% % \begin{center}
% \centering%
% \vspace{7pt}
%     \jsubfig{\includegraphics[height=3.0cm]{latex/images/distributions/smiling/paired/smiling_paired_test_-_not_smiling.png}}
% 	{i}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=3.0cm]{latex/images/distributions/smiling/unpaired/smiling_unpaired_test_-_not_smiling.png}}
% 	{ii}%
% \\
% \vspace{7pt}
% 	\jsubfig{\includegraphics[height=3.0cm]{latex/imageWe show that the injection of implicit pairs into unpaired sets strengthens the mapping between the two domains and improves the compatibility of their distributionss/distributions/smiling/no_aug/smiling_no_augmentation_test_-_not_smiling.png}}
% 	{iii}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=3.0cm]{latex/images/distributions/smiling/natural_aug/smiling_natural_augmentation_test_-_not_smiling.png}}
% 	{iv}%
% \\
% \vspace{7pt}
% \hline
% 	\jsubfig{\includegraphics[height=3.0cm]{latex/images/distributions/smiling/pix2pix_atob/smiling_pix2pix_test_-_not_smiling.png}}
% 	{v}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=3.0cm]{latex/images/distributions/smiling/completely_paired/smiling_completely_paired_test_-_not_smiling.png}}
% 	{vi}%
% \\
% \vspace{3pt}
% % \end{center}
% \caption{Non-Smiling to Smiling test experiment distributions. i) Pseudo-paired augmentation. ii) Pseudo-unpaired augmentation iii) No augmentation iv) Natural augmentation v) Completely pseudo-paired with pix2pix architecture vi) Completely pseudo-paired with cyclegan architecture}

% \label{fig:not_smiling_test_distributions}
% \end{figure}

==> figures/distributions_smiling_test.tex <==
\begin{figure}
\centering%
    \jsubfig{
    \includegraphics[height=3cm]{images/distributions/smiling/testing/smiling_paired_test_smiling_happy_baseline_comparison.png}
    }
	{(a)}%
	\jsubfig{
	\includegraphics[height=3cm]{images/distributions/smiling/testing/smiling_pix2pix_btoa_test_smiling_happy_cyclegan_pix2pix.png}
	}
	{(b)}
% \\
\vspace{3pt}
\caption{ \textit{Smile removal} test result distributions. (a) Comparison of pseudo-paired augmentation in cyan and fitted ellipses for the baseline methods in red. (b) Distribution of test results when training Pix2Pix (in red) and CycleGAN (in cyan) with a 100\% pseudo-paired dataset}
\label{fig:smiling_test_distributions}
\end{figure}

==> figures/distributions_smiling_train.tex <==
\begin{figure}
    \jsubfig{\includegraphics[height=3cm]{images/distributions/smiling/training/smiling_openface.png}}
	{Space of identities}
	%
	\jsubfig{\includegraphics[height=3cm]{images/distributions/smiling/training/smiling_happy.png}}
	{Space of expressions}%
	
\vspace{3pt}
% \end{center}
\caption{Pseudo-pairs visualized on representations not related to the task (space of identities) and representations related to the task (space of expressions) for the  \textit{smile removal} task. Above we use PCA to visualize smiling (in orange), neutral (in black) and augmented (in fuchsia), training samples.}
\label{fig:smiling_train_distributions}
\end{figure}


==> figures/eyeglasses_basic_experiments.tex <==
% % 2x2 format on two columns
% \begin{figure}
% % \begin{center}
% \centering%
% % \vspace{7pt}
% \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008446_real_A_eyeglasses_2000_with_2000.png}}
% 	{}%
% 	%\hfill%
% 	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008446_fake_B_eyeglasses_2000_with_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008446_fake_B_eyeglasses_bonus_2000_with_2000_skipped_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008446_fake_B_uneyeglasses_2000_2000_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
%  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008446_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
% \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008508_real_A_eyeglasses_2000_with_2000.png}}
% 	{}%
% 	%\hfill%
% 	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008508_fake_B_eyeglasses_2000_with_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008508_fake_B_eyeglasses_bonus_2000_with_2000_skipped_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008508_fake_B_uneyeglasses_2000_2000_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
%  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008508_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
% % \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008574_real_A_eyeglasses_2000_with_2000.png}}
% % 	{}%
% % 	%\hfill%
% % 	\hspace{3pt}
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008574_fake_B_eyeglasses_2000_with_0_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008574_fake_B_eyeglasses_bonus_2000_with_2000_skipped_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008574_fake_B_uneyeglasses_2000_2000_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	%\hfill%
% %  	\hspace{3pt}
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008574_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% % 	{}%
% % \\
% % \vspace{7pt}
% \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008779_real_A_eyeglasses_2000_with_2000.png}}
% 	{}%
% 	%\hfill%
% 	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008779_fake_B_eyeglasses_2000_with_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008779_fake_B_eyeglasses_bonus_2000_with_2000_skipped_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008779_fake_B_uneyeglasses_2000_2000_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
%  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008779_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
% \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008838_real_A_eyeglasses_2000_with_2000.png}}
% 	{\small{Source}}%
% 	\hfill%
% 	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008838_fake_B_eyeglasses_2000_with_0_merged_eyeglasses4000_results.png}}
% 	{\small{baseline}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008838_fake_B_eyeglasses_bonus_2000_with_2000_skipped_merged_eyeglasses4000_results.png}}
% 	{\small{+natural}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008838_fake_B_uneyeglasses_2000_2000_merged_eyeglasses4000_results.png}}
% 	{\small{+unpaired}}%
%  	\hfill%
%  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/eyeglasses_basic/008838_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% 	{\small{+paired}}%
% \\
% \vspace{3pt}
% % \end{center}
% \caption{\emph{Eyeglass removal} results using different dataset configurations. Above we illustrate our randomly selected results (on the right) compared against three augmentation baselines, described in Section \ref{pseudo_pairs_subsection}}

% \label{fig:quality_eyeglasses}
% \end{figure}

==> figures/eyeglasses_loss_robustness.tex <==

% % 2x2 format on two columns
% \begin{figure}[]
% % \begin{center}
% \centering%
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008446_real_A_eyeglasses_2000_with_2000.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008446_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% 	{}%	
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008446_fake_B_eyeglasses_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008446_fake_B_eyeglasses_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008508_real_A_eyeglasses_2000_with_2000.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008508_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% 	{}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008508_fake_B_eyeglasses_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008508_fake_B_eyeglasses_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008574_real_A_eyeglasses_2000_with_2000.png}}
%     {}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008574_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% 	{}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008574_fake_B_eyeglasses_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008574_fake_B_eyeglasses_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008779_real_A_eyeglasses_2000_with_2000.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008779_fake_B_eyeglasses_2000_with_2000_merged_eyeglasses4000_results.png}}
% 	{}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008779_fake_B_eyeglasses_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008779_fake_B_eyeglasses_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008838_real_A_eyeglasses_2000_with_2000.png}}
% 	{\small{Source image}}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008838_fake_B_eyeglasses_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{\small{Full loss term}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008838_fake_B_eyeglasses_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{\small{No cycle loss}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/eyeglasses_loss_robustness/008838_fake_B_eyeglasses_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{\small{No Idt loss}}%
% \\
% \vspace{3pt}
% % \end{center}
% \caption{ \emph{Eyeglasses removal} loss robustness experiment}

% \label{fig:eyeglasses_loss_robustness}
% \end{figure}

==> figures/eyeglasses_scalability_experiments.tex <==
% % 2x2 format on two columns
% \begin{figure}
% % \begin{center}
% \centering%
% % \vspace{7pt}
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008446_real_A_eyeglasses_10000_with_10000.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008446_fake_B_eyeglasses_10000_with_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008446_fake_B_uneyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% 	{}%
% % 	\hspace{3pt}
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008446_fake_B_eyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008508_real_A_eyeglasses_10000_with_10000.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008508_fake_B_eyeglasses_10000_with_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008508_fake_B_uneyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% 	{}%
% % 	\hspace{3pt}
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008508_fake_B_eyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008574_real_A_eyeglasses_10000_with_10000.png}}
% % 	{}%
% % 	\hfill%
% % 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008574_fake_B_eyeglasses_10000_with_0_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008574_fake_B_uneyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008574_fake_B_eyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% % 	{}%
% % \\
% % \vspace{7pt}
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008779_real_A_eyeglasses_10000_with_10000.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008779_fake_B_eyeglasses_10000_with_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008779_fake_B_uneyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% %  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008779_fake_B_eyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008838_real_A_eyeglasses_10000_with_10000.png}}
% 	{\small{Source}}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008838_fake_B_eyeglasses_10000_with_0_merged_eyeglasses4000_results.png}}
% 	{\small{baseline}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008838_fake_B_uneyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% 	{\small{+unpaired}}%
% % 	\hspace{3pt}
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/eyeglasses_scalability/008838_fake_B_eyeglasses_10000_with_10000_merged_eyeglasses4000_results.png}}
% 	{\small{+paired}}%
% \\
% \vspace{3pt}
% % \end{center}
% \caption{Scalabilty experiments on the \emph{eyeglass removal} task. Above we illustrate our randomly selected results (on the right) compared against two augmentation baselines, when trained on a larger dataset. As the figure demonstrates, augmenting with pseudo-pairs is beneficial for larger datasets as well. } 

% \label{fig:eyeglasses_scalability}
% \end{figure}

==> figures/first_stage_results_old.tex <==

%   \begin{table*}
  
% \centering
% \ra{1.0}
% \setlength{\tabcolsep}{2.35pt}
% \begin{tabular}{@{}ll cccccccccc cccccccccc@{}}
% \toprule{}
% \multicolumn{2}{c}{} &&  \multicolumn{8}{c}{\textbf{Reconstruction Loss}} & & \phantom{}  & \multicolumn{8}{c}{\textbf{FID Score}} \\
% \multicolumn{2}{c}{} &  & \multicolumn{2}{c}{$Cityscapes$} & \phantom{}& \multicolumn{2}{c}{$CVC-14$} & \phantom{}& \multicolumn{2}{c}{$Facades$}  & \phantom{}  & \phantom{}  & \multicolumn{2}{c}{$Cityscapes$} & \phantom{}& \multicolumn{2}{c}{$CVC-14$} & \phantom{}& \multicolumn{2}{c}{$Facades$} & \phantom{}  \\ \alpha
%       && & A2B   & B2A   &&  A2B  & B2A   && A2B   & B2A 
%       && & A2B   & B2A   &&  A2B  & B2A   && A2B   & B2A \\
%       \midrule{}
%   0 && & 0.270 & 0.169 && 0.134 & 0.159 && 0.365 & 0.820 
%       && & 1.109 & 1.124 && 1.168 & 1.150 && \textbf{1.047} & 1.044 \\  
%  0.25 && & 0.265 & 0.173 && 0.124 & 0.155 && 0.370 & 0.773
%       && & 1.106 & 1.126 && \textbf{1.143} & \textbf{1.147} && 1.053 & 1.046 \\ 
%  0.5 && & \textbf{0.244} & 0.170 && 0.122 & 0.151 && 0.390 & \textbf{0.735}
%       && & \textbf{1.096} & 1.126 && 1.157 & 1.155 && \textbf{1.047} & 1.040 \\
%  0.75 && & 0.249 & \textbf{0.163} && \textbf{0.118} & \textbf{0.149} && \textbf{0.350} & 0.744  
%       && & 1.107 & \textbf{1.119} && 1.156 & 1.150 && 1.055 & \textbf{1.032} \\
% 1 && & 0.259 & 0.167 && 0.130 & 0.152 && 0.375 & 0.740
%       && & 1.105 & 1.150 && 1.152 & 1.154 && 1.062 & 1.034 \\  
%       \midrule{}
% Pix2pix && & 0.267 & 0.216 && 0.092 & 0.344 && 0.33 & 0.263
%       && & 1.106 & 1.107 && 1.087 & 1.079 && 1.029 & 1.053 \\  

% \bottomrule{}
% \end{tabular}
% %\footnotesize
% 	\caption{Comparison of reconstruction loss and FID score over several pairing ratios. Remarkably there is not a single instance where complete pairing is the best option.}
% 	\label{table:first_stage_results}
% \end{table*}


==> figures/pix2pix_results.tex <==

%   \begin{table*}
%   \label{tab:first_stage_results}
% \centering
% \ra{1.0}
% \setlength{\tabcolsep}{2.35pt}
% \begin{tabular}{@{}ll cccccccccc cccccccccc@{}}
% \toprule{}
% \multicolumn{2}{c}{} &  &  \multicolumn{8}{c}{\textbf{Reconstruction Loss}} && \phantom{}  & \multicolumn{8}{c}{\textbf{FID Score}} \\
% \multicolumn{2}{c}{} &  & \multicolumn{2}{c}{$Cityscapes$} & \phantom{}& \multicolumn{2}{c}{$CVC-14$} & \phantom{}& \multicolumn{2}{c}{$Facades$}  & \phantom{}  & \phantom{}  & \multicolumn{2}{c}{$Cityscapes$} & \phantom{}& \multicolumn{2}{c}{$CVC-14$} & \phantom{}& \multicolumn{2}{c}{$Facades$} & \phantom{}  \\ \alpha
%       && & A2B   & B2A   &&  A2B  & B2A   && A2B   & B2A 
%       && & A2B   & B2A   &&  A2B  & B2A   && A2B   & B2A \\
%       \midrule{}
%   0 && & 0.270 & 0.169 && 0.134 & 0.159 && 0.365 & 0.820 
%       && & 1.109 & 1.124 && 1.168 & 1.150 && \textbf{1.047} & 1.044 \\  
%  0.25 && & 0.265 & 0.173 && 0.124 & 0.155 && 0.370 & 0.773
%       && & 1.106 & 1.126 && \textbf{1.143} & \textbf{1.147} && 1.053 & 1.046 \\ 
%  0.5 && & \textbf{0.244} & 0.170 && 0.122 & 0.151 && 0.390 & \textbf{0.735}
%       && & \textbf{1.096} & 1.126 && 1.157 & 1.155 && \textbf{1.047} & 1.040 \\
%  0.75 && & 0.249 & \textbf{0.163} && \textbf{0.118} & \textbf{0.149} && \textbf{0.350} & 0.744  
%       && & 1.107 & \textbf{1.119} && 1.156 & 1.150 && 1.055 & \textbf{1.032} \\
% 1 && & 0.259 & 0.167 && 0.130 & 0.152 && 0.375 & 0.740
%       && & 1.105 & 1.150 && 1.152 & 1.154 && 1.062 & 1.034 \\  

% \bottomrule{}
% \end{tabular}
% %\footnotesize
% 	\caption{Comparison of reconstruction loss and FID score over several pairing ratios. Remarkably there is not a single instance where complete pairing is the best option.}
% \end{table*}


==> figures/pix2pix_vs_cyclegan.tex <==

% \begin{table}[h!]
% \centering
% \begin{tabular}{ |p{1.5cm}||p{1.3cm}|p{1.3cm}|p{1.3cm}|p{1.3cm}|  }
%  \hline
%  \multirow{Training Regime} & \multicolumn{2}{c|}{A2B} & \multicolumn{2}{c|}{B2A}\\
%  \cline{2-5} 
% & Reconstruction & FID & Reconstruction & FID \\
% \hline
%  0\%     & 0.27           & 1.109          & 0.169          & 1.124 \\
%  \hline
%  100\%   & 0.259          & \textbf{1.105} & \textbf{0.167} & 1.15 \\
%  \hline
%  Pix2Pix & \textbf{0.089} & 1.111 & 0.216  & \textbf{1.13} \\
%  \hline
% \end{tabular}
% \caption{Explicit vs. Implicit training with Cityscapes: Comparison of training with Pix2Pix vs. CycleGAN}
% \label{table:pix2pix_vs_cyclegan}
% \end{table}


==> figures/smiling_basic_experiments.tex <==

% % 2x2 format on two columns
% \begin{figure}
% % \begin{center}
% \centering%
% % \vspace{7pt}
% %     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002317_real_A_smiling_paired_2000_2000_a2.png}}
% % 	{}%
% % 	\hfill%
% % 	\hspace{3pt}
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002317_fake_B_smiling_paired_2000_0_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002317_fake_B_smiling_bonus_skipped_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002317_fake_B_unsmiling_2000_with_2000_a2_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% %  	\hspace{3pt}
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002317_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% % 	{}%
% % \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002350_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hfill%
% 	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002350_fake_B_smiling_paired_2000_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002350_fake_B_smiling_bonus_skipped_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002350_fake_B_unsmiling_2000_with_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
%  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002350_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002354_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hfill%
% 	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002354_fake_B_smiling_paired_2000_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002354_fake_B_smiling_bonus_skipped_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002354_fake_B_unsmiling_2000_with_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
%  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002354_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002367_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hfill%
% 	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002367_fake_B_smiling_paired_2000_0_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002367_fake_B_smiling_bonus_skipped_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002367_fake_B_unsmiling_2000_with_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
%  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002367_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002377_real_A_smiling_paired_2000_2000_a2.png}}
% 	{\small{source}}%
% 	\hfill%
% 	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002377_fake_B_smiling_paired_2000_0_merged_eyeglasses4000_results.png}}
% 	{\small{baseline}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002377_fake_B_smiling_bonus_skipped_merged_eyeglasses4000_results.png}}
% 	{\small{+natural}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002377_fake_B_unsmiling_2000_with_2000_a2_merged_eyeglasses4000_results.png}}
% 	{\small{+unpaired}}%
%  	\hfill%
%  	\hspace{3pt}
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_basic/002377_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{\small{+paired}}%
% \\
% \vspace{3pt}
% % \end{center}
% \caption{Results for the  \emph{smile removal} task using different dataset configurations. Above we illustrate our randomly selected results (on the right) compared against three augmentation baselines, described in Section \ref{pseudo_pairs_subsection}.
%  }

% \label{fig:quality_smiling}
% \end{figure}

==> figures/smiling_loss_robustness.tex <==

% % 2x2 format on two columns
% \begin{figure}[]
% % \begin{center}
% \centering%
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002317_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002317_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%	
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002317_fake_B_smiling_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002317_fake_B_smiling_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002350_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002350_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002350_fake_B_smiling_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002350_fake_B_smiling_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002354_real_A_smiling_paired_2000_2000_a2.png}}
%     {}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002354_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002354_fake_B_smiling_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}} 
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002354_fake_B_smiling_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002367_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002367_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002367_fake_B_smiling_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002367_fake_B_smiling_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% \vspace{7pt}
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002377_real_A_smiling_paired_2000_2000_a2.png}}
% 	{\small{Source image}}%
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002377_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{\small{Full loss term}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002377_fake_B_smiling_2000_with_2000_signaling_cycleloss_merged_eyeglasses4000_results.png}}
% 	{\small{No cycle loss}}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.6cm]{latex/images/experiment_folders/smiling_loss_robustness/002377_fake_B_smiling_2000_with_2000_signaling_idtloss_merged_eyeglasses4000_results.png}}
% 	{\small{No Idt loss}}%
% \\
% \vspace{3pt}
% % \end{center}
% \caption{Smiling loss robustness experiment}

% \label{fig:smiling_loss_robustness}
% \end{figure}

==> figures/smiling_pairing_ratio_experiments.tex <==
% % 2x2 format on two columns
% \begin{figure}
% % \begin{center}
% \centering%
% % \vspace{7pt}
% %     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002317_real_A_smiling_paired_2000_2000_a2.png}}
% % 	{}%
% % 	\hfill%
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002317_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002317_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002317_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002317_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% % 	{}%
% % \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002350_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002350_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}}
% 	{}%
% % 	\hspace{3pt}
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002350_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002350_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002350_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002354_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002354_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}}
% 	{}%
% % 	\hspace{3pt}
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002354_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002354_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002354_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002367_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002367_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}}
% 	{}%
% % 	\hspace{3pt}
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002367_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002367_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002367_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002377_real_A_smiling_paired_2000_2000_a2.png}}
% 	{\small{source}}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002377_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}}
% 	{\small{25\% }}%
% % 	\hspace{3pt}
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002377_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{\small{50\% }}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002377_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}}
% 	{\small{90\% }}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=1.55cm]{latex/images/experiment_folders/smiling_pairing_ratio/002377_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}}
% 	{\small{100\% }}%
% \\
% \vspace{3pt}
% % \end{center}
% \caption{Pseudo-pair ratio analysis for the  \emph{smile removal} task. Above we illustrate a few randomly selected results using various pairing ratios. As the figure illustrates, using a 50\% pairing configuration yields identity-preserving results which perform the task (smile removal in this case) better than a higher pairing ratio.  }

% \label{fig:smiling_pairing_ratios}
% \end{figure}

==> figures/smiling_training_regimes.tex <==

% % 2x2 format on two columns
% \begin{figure}
% % \begin{center}
% \centering%
% % \vspace{7pt}
% %     \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002317_real_A_smiling_paired_2000_2000_a2.png}}
% % 	{}%
% % 	\hfill%
% % 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002317_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002317_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}}
% % 	{}%
% %  	\hfill%
% % 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002317_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}}
% % 	{}%
% % \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002350_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002350_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002350_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002350_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002354_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002354_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002354_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002354_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002367_real_A_smiling_paired_2000_2000_a2.png}}
% 	{}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002367_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002367_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}}
% 	{}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002367_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}}
% 	{}%
% \\
% % \vspace{7pt}
%     \jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002377_real_A_smiling_paired_2000_2000_a2.png}}
% 	{\small{Source }}%
% 	\hspace{3pt}
% 	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002377_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}}
% 	{\small{Implicit }}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002377_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}}
% 	{\small{Explicit }}%
%  	\hfill%
% 	\jsubfig{\includegraphics[height=2.0cm]{latex/images/experiment_folders/smiling_training_regimes/002377_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}}
% 	{\small{Semi-explicit}}%
% \\
% \vspace{3pt}
% % \end{center}
% \caption{\emph{Smile removal} with pseudo-pairs in different settings. Above we illustrate a few randomly selected results by models trained using either an explicit (\cite{DBLP:journals/corr/IsolaZZE16}), semi-explicit (\cite{DBLP:journals/corr/abs-1805-03189}), or implicit  (\cite{DBLP:journals/corr/ZhuPIE17}) settings.
% As the figure illustrates, an  implicit setting leads to the best and most consistent results.}

% \label{fig:smiling_training_regimes}
% \end{figure}

==> figures/tables/distribution_comparison.tex <==
% \begin{table}
% \centering
% \begin{tabular}{p{2.0cm}|p{1.0cm}p{1.0cm} } 

%  Parameter & 
%  \multicolumn{1}{c}{Pseudo-pair} & \multicolumn{1}{c}{Mean baseline}
%  \\
% \hline
%  x & \textbf{0.27} & 1.37 \\
%  y &  \textbf{0.02} & 0.05 \\
%  Major axis &  \textbf{0.27}  & 5.65 \\
%  Minor axis &  \textbf{0.03} & 0.04
 
% \end{tabular}
% \caption{Comparison of MSE between the ellipse fitted to non-smiling samples and ellipse fitted on samples generated with the pseudo-pair augmentation method (in cyan) and the mean MSE between the ellipse fitted to non-smiling samples and the ellipse fitted by the baseline methods (in red). Lower is better.}
% \label{table:distribution_ellipse_comparison}
% \end{table}

==> figures/tables/eyeglasses_scalability_table.tex <==
% \begin{table}
% \centering
% \begin{tabular}{ p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm} }
% %  \hline
%  \multicolumn{1}{c}{0-Paired} & \multicolumn{1}{c}{0.25-Paired} & \multicolumn{1}{c}{0.5-Paired}
%  & \multicolumn{1}{c}{0.75-Paired} & \multicolumn{1}{c}{1-Paired} \\
% \hline
% 0.00242 & 0.00199 & 0.00152 & 0.00109 & \textbf{0.000127} \\
% %  \hline
% \end{tabular}
% \caption{$\texttt{InfoSim}$ values for scalability experiments on the  \emph{Eyeglass removal} task. Lower is better.}
% \label{table:scalability_identity_preservation}
% \end{table}

==> figures/tables/foggy_fcn8.tex <==
% % \vspace{-2mm}
% \begin{table}
% \centering
% \begin{tabular}{ p{1.4cm} p{1.0cm} p{1.0cm} p{1.0cm} } 
% %  \hline
% $\alpha$ & 
%  \multicolumn{1}{c}{\textbf{Per-pixel acc.}} & \multicolumn{1}{c}{\textbf{Per-class acc.}}
%  & \multicolumn{1}{c}{\textbf{Class IOU}} \\
% \hline
%  0 & 0.523 & 0.189 & 0.111 \\
%  0.25 & 0.549 & 0.197 & 0.117 \\
%  0.5 & 0.550 & 0.200 & 0.121 \\
%  0.75 & 0.572 & 0.202 & 0.126 \\
%  1  & \textbf{0.576} & \textbf{0.204} & \textbf{0.128}
% %  \hline
 
% \end{tabular}
% \caption{FCN-scores for different implicit pairing ratios, $\alpha$ on Foggy Cityscapes dataset, higher is better.}
% \label{table:foggy_fcn8}
% \end{table}

==> figures/tables/smiling_training_regimes_table.tex <==
\begin{table}
\centering
\begin{tabular}{ p{1.3cm}p{1.3cm} }
%  \hline
%  \multicolumn{4}{|c|}{Smiling parameter search: Identity conservation distance} \\
%  \hline
 \multicolumn{1}{c}{Implicit} & \multicolumn{1}{c}{Explicit} \\
\hline
 0.00180    & \textbf{0.000342} \\
%  \hline
\end{tabular}
\caption{\texttt{InfoSim} values for explicit and implicit experiments on the  \emph{Eyeglass removal} task. Lower is better.}
\label{table:training_regimes_identity_preservation}
\end{table}

==> includes/algorithms.tex <==

% \begin{algorithm}[t]
% \caption{Learning in Paired Setting}
% % \label{alg}
% \begin{algorithmic}
% \STATE \textbf{Input:} A paired dataset $(A, B)$. 	
% \STATE \textbf{Output:} $G_{AB}$ and $G_{BA}$.
% \FOR{each epoch }
% \STATE Sample pairs $(a,b) \in \{A, B\}$
% \STATE Update model in respect to:
% \STATE \hspace{10pt} $L(G_{AB},G_{BA}, D_A, D_B, a, b)$
% \ENDFOR
% % \COMMENT{\todo{The sampling notation isn't tight enough}}
% \end{algorithmic}
% \label{alg_explicit}
% \end{algorithm}

% \begin{algorithm}
% \caption{Learning in Unpaired Setting}
% % \label{alg}
% \begin{algorithmic}
% \STATE \textbf{Input:} An unpaired dataset $(A, B)$. 	
% \STATE \textbf{Output:} $G_{AB}$ and $G_{BA}$.
% \FOR{each epoch }
% \STATE Sample $a \in A, b \in B$
% \STATE Update model in respect to:
% \STATE \hspace{10pt} $L_{AB}(G_{AB},G_{BA}, D_B, a)$
% \STATE \hspace{15pt}$ + L_{BA}(G_{AB},G_{BA}, D_A, b)$
% \ENDFOR
% % \COMMENT{\todo{The sampling notation isn't tight enough}}
% \end{algorithmic}
% \label{alg_implicit}
% \end{algorithm}

==> pseudo_experiments/scalability.tex <==

% \input{latex/figures/tables/eyeglasses_scalability_table.tex}

% \input{latex/figures/eyeglasses_scalability_experiments.tex}

% \paragraph{Scalability experiments.}
% % \vspace{-0.7em}
% Data augmentation is usually most effective when the size of the dataset is small and correspondingly our experiments were done with very small datasets (up to 4000 samples). We are interested in understanding whether learning with implicit pseudo-pairs is still beneficial with larger datasets. To accomplish this we repeat the basic experiments with datasets that are 5 times larger. Due to limits in the celebA dataset in these experiments we have 10K samples in each domain with additional 10K augmentation samples. Due to these restrictions we are also unable to repeat the \emph{natural} augmentation experiment.
% The results shown in Table \ref{table:scalability_identity_preservation} and Figure \ref{fig:eyeglasses_scalability} demonstrate that pseudo-pairs lead to impressive improvements even in large datasets.

==> supplamentary.tex <==
\input{supplamentary/text.tex}


\input{supplamentary/cityscapes_results.tex}

% \section{Pseudo-pairs results}

\input{supplamentary/baseline_results.tex}


\input{supplamentary/ratio_results.tex}

\input{supplamentary/settings_results.tex}

==> supplamentary/ratio_results/smiling_qualitative_old.tex <==



% \begin{figure}
%   \centering% 
 


% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001411_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001411_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001411_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001411_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001411_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001424_real_A_smiling_paired_2000_2000_a2.png}} 
% %  {}% 
% % \hspace{3pt}
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001424_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001424_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001424_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001424_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001504_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001504_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001504_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001504_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001504_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001516_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001516_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001516_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001516_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001516_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001536_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001536_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001536_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001536_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/001536_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003523_real_A_smiling_paired_2000_2000_a2.png}} 
% %  {}% 
% % \hspace{3pt}
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003523_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003523_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003523_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003523_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \\  

% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003529_real_A_smiling_paired_2000_2000_a2.png}} 
% %  {}% 
% % \hspace{3pt}
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003529_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003529_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003529_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003529_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003584_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003584_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003584_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003584_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003584_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003588_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003588_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003588_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003588_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003588_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003615_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003615_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003615_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003615_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/003615_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002654_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002654_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002654_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002654_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002654_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002655_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002655_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002655_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002655_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002655_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002661_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002661_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002661_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002661_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002661_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002728_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002728_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002728_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002728_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002728_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002745_real_A_smiling_paired_2000_2000_a2.png}} 
%  {Source}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002745_fake_B_smiling_2000_with_2000_ratio_05_merged_eyeglasses4000_results.png}} 
%  {25\%}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002745_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {50\%}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002745_fake_B_smiling_2000_with_2000_asize_200_merged_eyeglasses4000_results.png}} 
%  {90\%}% 
% \hfill%
% \jsubfig{\includegraphics[height=1.6cm]{latex/images/supplamentary/ratio_results/smiling_parameters_pairing_ratio_experiment/002745_fake_B_smiling_2000_with_2000_asize_0_merged_eyeglasses4000_results.png}} 
%  {100\%}% 
% \hfill%
% \vspace{3pt} 
 
%  \caption{Additional random pseudo-pair ratio analysis results for the  \emph{smile removal} task} 
%  \end{figure} 


==> supplamentary/training_regimes/smiling_training_regimes_old.tex <==



% \begin{figure}
%   \centering% 
 
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018822_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018822_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018822_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018822_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018841_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018841_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018841_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018841_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018875_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018875_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018875_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018875_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018877_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018877_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018877_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018877_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018881_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018881_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018881_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/018881_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022075_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022075_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022075_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022075_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022076_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022076_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022076_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022076_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022089_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022089_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022089_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022089_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022118_real_A_smiling_paired_2000_2000_a2.png}} 
%  {}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022118_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022118_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022118_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {}% 
% \hfill%
% \\  



% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022131_real_A_smiling_paired_2000_2000_a2.png}} 
%  {Source}% 
% \hspace{3pt}
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022131_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
%  {Implicit}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022131_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
%  {Explicit}% 
% \hfill%
% \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/022131_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
%  {Semi-explicit}% 
% \hfill%
% \\  



% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010863_real_A_smiling_paired_2000_2000_a2.png}} 
% %  {}% 
% % \hspace{3pt}
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010863_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010863_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010863_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \\  



% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010887_real_A_smiling_paired_2000_2000_a2.png}} 
% %  {}% 
% % \hspace{3pt}
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010887_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010887_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010887_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \\  



% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010909_real_A_smiling_paired_2000_2000_a2.png}} 
% %  {}% 
% % \hspace{3pt}
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010909_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010909_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010909_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \\  



% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010934_real_A_smiling_paired_2000_2000_a2.png}} 
% %  {}% 
% % \hspace{3pt}
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010934_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010934_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010934_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \\  



% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010939_real_A_smiling_paired_2000_2000_a2.png}} 
% %  {}% 
% % \hspace{3pt}
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010939_fake_B_smiling_paired_2000_2000_a2_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010939_fake_B_smiling_2000_with_2000_pix2pix_atob_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% % \jsubfig{\includegraphics[height=2.0cm]{latex/images/supplamentary/training_regimes/smiling_parameters_training_regimes_experiment/010939_fake_B_smiling_2000_with_2000_implicitfirst_merged_eyeglasses4000_results.png}} 
% %  {}% 
% % \hfill%
% \vspace{3pt} 
 
%  \caption{Additional random \emph{Smile removal} results with pseudo-pairs in different settings.} 
%  % \label{} 
%  \end{figure} 
